Reach-SDP: Reachability Analysis of Closed-Loop Systems with Neural Network Controllers via Semidefinite Programming

There has been an increasing interest in using neural networks in closed-loop control systems to improve performance and reduce computational costs for on-line implementation. However, providing safety and stability guarantees for these systems is challenging due to the nonlinear and compositional structure of neural networks. In this paper, we propose a novel forward reachability analysis method for the safety verification of linear time-varying systems with neural networks in feedback interconnection. Our technical approach relies on abstracting the nonlinear activation functions by quadratic constraints, which leads to an outer-approximation of forward reachable sets of the closed-loop system. We show that we can compute these approximate reachable sets using semidefinite programming. We illustrate our method in a quadrotor example, in which we first approximate a nonlinear model predictive controller via a deep neural network and then apply our analysis tool to certify finite-time reachability and constraint satisfaction of the closed-loop system.

==> contents/batch.tex <==
\subsection{Batch Reach-SDP}
In this subsection, we introduce the \textit{Batch Reach-SDP}, which approximates the $N$-step reachable set $\Reach^N(\init)$ by solving only one single SDP problem,
\begin{equation}
\begin{aligned}
\label{eq::batch_SDP}
\ReachBar^{N}(\init) &= \operatorname{Batch\_Reach\_{SDP}}\left(\init\right).
\end{aligned}
\end{equation}
The key idea here is that we abstract the neural network controllers $\nnc(x(\tau)), \ \tau = 0,\cdots,N-1$ with relaxed networks $\absnnc(x(\tau))$ described by $N$ different QCs.
Therefore, we consider the following basis vector:
\begin{equation}
\label{eq::batch_basis}
    [\hbx^\top \ 1]^\top \coloneqq [x_0^\top \ {\bx_0}^\top \ \cdots \ {\bx_{N-1}}^\top \ 1]^\top \in \R^{n_x+N n_n+1}
\end{equation}
where $\bx_\tau \coloneqq [{x_\tau^1}^\top \ \cdots \ {x_\tau^\ell}^\top]^\top \in \R^{n_n}$ describes the neurons in the abstracted neural network $\absnnc(x(\tau))$ at time $\tau$.
The following theorem provides a sufficient condition for over-approximating the $N$-step reachable set $\Reach^N(\init)$ of the closed-loop system \eqref{eq::closed_loop_sys}.

\begin{theorem}[SDP for $N$-step reachable set]
\label{thm::eq::batch_SDP}
Consider the closed-loop system \eqref{eq::closed_loop_sys}.
Suppose the initial set $\init$ satisfies the QCs defined by
\begin{equation}
\label{eq::batch_SDP::input}
\left\{ \bMin \,\middle\vert\, \bMin = \bEin^\top P \bEin \geq 0 \right\},
\end{equation}
with the change-of-basis matrix,
\begin{equation}
\bEin = \begin{bmatrix}
I_{n_x} &0 &\cdots &0 &0 \\
0 &0 &\cdots &0 &1
\end{bmatrix},
%\in \R^{n_x+1 \times n_x+N n_n+1}
\end{equation}
and the neural network controllers $\nnc(x(\tau))$ satisfy the QCs defined by
\begin{equation}
\begin{aligned}
\label{eq::batch_SDP::mid}
\left\{ \bMmid \,\middle\vert\, \bMmid = \bEmid^\top \Mmid(Q_\tau) \bEmid \geq 0 \right\}
\end{aligned}
\end{equation}
where $\Mmid(Q_\tau) \subseteq \R^{n_x+n_n+1}$ is defined in Proposition \ref{prop::mid} and the change-of-basis matrix is,
\begin{equation}
\begin{aligned}
&\bEmid = \\
&\begin{bmatrix}
\displaystyle\prod_{i=0}^\tau A_i  &0 &\displaystyle\prod_{i=0}^{\tau-1} A_i B_0 W^\ell &\cdots &B_\tau W^\ell &0 &\cdots &C_\tau \\
0 &0 &\cdots &0 &0 &I_{n_n} &\cdots &0 \\
0 &0 &\cdots &0 &0 &0 &\cdots &1
\end{bmatrix}
\end{aligned}
\end{equation}
where $C_\tau = \sum_{i=0}^{\tau-1} A^{\tau-i-1} (B_i b^\ell + c_i)$.
Suppose also the saturated neural network control inputs $\sat(\nnc(x(\tau)))$ satisfy the QCs defined by
\begin{equation}
\begin{aligned}
\label{eq::batch_SDP::mid}
\left\{ \bMproj \,\middle\vert\, \bMproj = \bEproj^\top \Mproj(O_\tau) \bEproj \geq 0 \right\}
\end{aligned}
\end{equation}
where $\Mproj(O_\tau) \subseteq \R^{n_x+n_n+1}$ is defined in Proposition \ref{prop::proj} and the change-of-basis matrix is,
\begin{equation}
\begin{aligned}
&\bEproj = \begin{bmatrix}
0 &\cdots &0 &W^\ell &0 &\cdots &0 &b^\ell \\
0 &\cdots &0 &0 &0 &\cdots &0 &1 
\end{bmatrix}.
\end{aligned}
\end{equation}
Let the candidate set $\ReachBar^N(\init)$ satisfy the quadratic inequality defined by
\begin{equation}
\begin{aligned}
\label{eq::batch_SDP::out}
\left\{ \hbx \in \R^{n_x+N n_n}  \,\middle\vert\, \begin{bmatrix} \hbx \\ 1\end{bmatrix}^\top \underbrace{\bEout^\top S \bEout}_{\bMout(S)} \begin{bmatrix} \hbx \\ 1\end{bmatrix} \leq 0 \right\}
\end{aligned}
\end{equation}
with the change-of-basis matrix,
\begin{equation}
\begin{aligned}
&\bEout = \\
&\begin{bmatrix}
\displaystyle\prod_{i=0}^{N-1} A_i  &0 &\displaystyle\prod_{i=0}^{N-2} A_i B_0 W^\ell &\cdots &B_{N-1} W^\ell  &C_N \\
0 &0 &0 &\cdots &0 &1
\end{bmatrix}.
\end{aligned}
\end{equation}
If the following LMI
\begin{equation}
\label{lmi::eq::batch_SDP}
    \bMin(P) + \bMout(S) + \sum_{\tau=0}^{N-1} \bMmid(Q_\tau) + \bMproj(O_\tau)  \preceq 0,
\end{equation}
is feasible for some matrices $(P,\{Q_\tau\}_{\tau=0}^{N-1},\{O_\tau\}_{\tau=0}^{N-1},S) \in \mathcal{P} \times \mathcal{Q}^N \times \mathcal{O}^N \times \Sym^{n_x+1}$, then $\Reach^N(\init) \subseteq \ReachBar^N(\init)$.
\end{theorem}

\begin{proof}
Follows the proof of Theorem \ref{thm::seq_sdp}.
\end{proof}

\vspace{5pt}

\noindent Similar to \eqref{sdp::poly} and \eqref{sdp::ellips}, we can formulate an SDP problem to minimize the volume of the $N$-step approximate reachable set $\ReachBar^N(\init)$ with \eqref{lmi::eq::batch_SDP} as the constraint.
